DALLE-2 is Seeing Double: Flaws in Word-to-Concept Mapping in Text2Image Models

We study the way DALLE-2 maps symbols (words) in the prompt to their references (entities or properties of entities in the generated image). We show that in stark contrast to the way human process language, DALLE-2 does not follow the constraint that each word has a single role in the interpretation, and sometimes re-use the same symbol for different purposes. We collect a set of stimuli that reflect the phenomenon: we show that DALLE-2 depicts both senses of nouns with multiple senses at once; and that a given word can modify the properties of two distinct entities in the image, or can be depicted as one object and also modify the properties of another object, creating a semantic leakage of properties between entities. Taken together, our study highlights the differences between DALLE-2 and human language processing and opens an avenue for future study on the inductive biases of text-to-image models.

==> tables/reference_leakage_challenge_table.tex <==
\begin{table*}[h]
\centering
\scalebox{0.85}{
\begin{tabular}{l|c}

    \hline
    Challenge & Modification Ratio \\
    \hline\hline
     An \textbf{armadillo} on a \textit{sea} shore\footnote{Armadillos have a \textbf{shell}, the prompt results in an image of an armadillo on a seashore with seashells.} & 12/12  \\
     \hline
     A \textbf{pinniped} is opening a \textit{letter} & 7/12 \\
     \hline
     a person \textbf{jaywalking} and a \textit{bird} & 11/12 \\
     \hline
     a \textbf{tall, long-legged, long-necked bird} and a \textit{construction site} & 12/12 \\
     \hline
     \textit{food} and a \textbf{cone} hat, zoomed out photo & 12/12 \\
     \hline
     A \textbf{zebra} and a \textit{street} & 10/12 \\
     \hline
     A \textbf{seal} is opening a \textit{letter} & 10/12 \\
     \hline
     Two people play \textbf{squash} with \textit{food} & 12/12 \\
     \hline
     a \textbf{pool} and a \textit{table} & 10/12 \\
     \hline
     A \textit{fish} and a \textbf{gold} ingot & 12/12 \\
     \hline
     A \textbf{cup} in a bakery with \textit{cakes} & 11/12 \\
     \hline
     An \textit{animal} alongside a \textbf{piggy bank} & 12/12 \\
     \hline
     A \textbf{basketball} near \textit{groceries} & 12/12 \\
     \hline
     A \textbf{cross} and a \textit{sidewalk} & 10/12 \\
     \hline
     A \textbf{ladybug} and a \textit{person}, full body image & 11/12 \\
     \hline
     A \textbf{leopard} and a \textit{piece of cloth} & 11/12 \\
     \hline
     \textbf{peanuts} and \textit{classic butter} & 12/12 \\
     \hline
     A \textit{person} and a \textbf{bug with red spots}, full body image & 11/12 \\
     \hline
    \end{tabular}
    }
    \caption{Detailed table for Challenge Prompts in \textbf{Reference Leakage}, modifier nouns are denoted with \textbf{bold}, modified nouns are denoted with \textit{italic} \shauli{can we replace the challenge and control tables with 1 longer table where each cell is sub-divided into two boxes, ``challenge" and ``control"? it's much easier to read that way}}
\end{table*}

==> tables/reference_leakage_control_table.tex <==
\begin{table*}[h]
\centering
\scalebox{0.85}{
\begin{tabular}{l|c}
    \hline
    Control & Modification Ratio \\
    \hline\hline
     A dog on a sea shore & 0/12  \\
     \hline
     A large water mammal is opening a letter\footnote{\textit{A large water mammal is opening a letter} is a control prompt for \textit{A pinniped is opening a letter} and \textit{A seal is opening a letter}} & 1/12 \\
     \hline
     A person crossing the street unlawfully and a bird & 0/12 \\
     \hline
     a bird and a construction site & 0/12 \\
     \hline
     food and a birthday hat, zoomed out photo & 0/12 \\
     \hline
     a zebra and a gravel street & 0/12 \\
     \hline
     Two people play squash & 0/12 \\
     \hline
     a pool and a bar & 0/12 \\
     \hline
     A fish and an ingot & 0/12 \\
     \hline
     A cup in a bakery & 0/12 \\
     \hline
     An animal alongside a table & 0/12 \\
     \hline
     A football near groceries & 5/12 \\
     \hline
     a crucifix and a sidewalk & 2/12 \\
     \hline
     A bug and a person, full body image\footnote{\textit{A bug and a person, full body image} is a control prompt for \textit{A ladybug and a person, full body image} and \textit{A person and a bug with red spots, full body image}} & 6/12 \\
     \hline
     a leopard and a black towel & 5/12 \\
     \hline
     cucumbers and classic butter & 0/12 \\
     \hline
    \end{tabular}
    }
    \caption{Detailed table for Control prompts in \textbf{Reference Leakage}}
\end{table*}

==> title_page.tex <==
\title{DALLE-2 is Seeing Double: Flaws in Word-to-Entity Mapping
}

 \author{Royi Rassin$\footnotemark[1]$ \textsuperscript{{ \normalfont 1}}, Shauli Ravfogel$\thanks{~~Equal contribution.}$ \textsuperscript{{ \normalfont 1,2}} \, Yoav Goldberg\textsuperscript{\normalfont 1,2} \\
\textsuperscript{1}Bar-Ilan University \, \textsuperscript{2}Allen Institute for Artificial Intelligence \\
  {\tt\{\href{mailto:rassinroyi@gmail.com}{rassinroyi},
  \href{mailto:shauli.ravfogel@gmail.com}{shauli.ravfogel}, \href{mailto:yoav.goldberg@gmail.com}{yoav.goldberg}\}@gmail.com} 
  }
  

